Machine Learning Training on a Real Processing-in-Memory System

Training machine learning algorithms is a computationally intensive process, which is frequently memory-bound due to repeatedly accessing large training datasets. As a result, processor-centric systems (e.g., CPU, GPU) suffer from costly data movement between memory units and processing units, which consumes large amounts of energy and execution cycles. Memory-centric computing systems, i.e., computing systems with processing-in-memory (PIM) capabilities, can alleviate this data movement bottleneck. Our goal is to understand the potential of modern general-purpose PIM architectures to accelerate machine learning training. To do so, we (1) implement several representative classic machine learning algorithms (namely, linear regression, logistic regression, decision tree, K-means clustering) on a real-world general-purpose PIM architecture, (2) characterize them in terms of accuracy, performance and scaling, and (3) compare to their counterpart implementations on CPU and GPU. Our experimental evaluation on a memory-centric computing system with more than 2500 PIM cores shows that general-purpose PIM architectures can greatly accelerate memory-bound machine learning workloads, when the necessary operations and datatypes are natively supported by PIM hardware. To our knowledge, our work is the first one to evaluate training of machine learning algorithms on a real-world general-purpose PIM architecture.

==> UPMEM+ML - ISVLSI - arXiv-2/figures/tab-comparison.tex <==
\begin{tabular}{|l||l|l|}
\hline
\textbf{ML workload} & \textbf{CPU implementation} & \textbf{GPU implementation} \\
\hline
\hline
Linear regression & Intel MKL~\cite{mkl} & NVIDIA cuBLAS~\cite{cublas} \\ \hline
Logistic regression & Intel MKL~\cite{mkl} & NVIDIA cuBLAS~\cite{cublas} \\ \hline
Decision tree & Scikit-learn~\cite{pedregosa2011scikit} & RAPIDS~\cite{rapids} \\ \hline
Kmeans & Scikit-learn~\cite{pedregosa2011scikit} & RAPIDS~\cite{rapids} \\ \hline
\end{tabular}


==> UPMEM+ML - ISVLSI - arXiv-2/figures/tab-cpugpu.tex <==
\begin{tabular}{|l||c|ccc|cc|c|}
\hline
\multirow{2}{*}{\textbf{System}} & \textbf{Process} & \multicolumn{3}{c|}{\textbf{Processor Cores}} & \multicolumn{2}{c|}{\textbf{Memory}} & \multirow{2}{*}{\textbf{TDP}} \\
\cline{3-7}
& \textbf{Node} & \textbf{Total Cores} & \textbf{Frequency} & \textbf{Peak Performance} & \textbf{Capacity} & \textbf{Total Bandwidth} & \\
\hline
\hline
\textbf{UPMEM PIM System}~\cite{upmem} & 2x nm & 2,560$^\diamond$ & 425 MHz & 1,088 GOPS & 160 GB & 2.1 TB/s & 280 W$^\dagger$ \\ \hline
\textbf{Intel Xeon Silver 4215 CPU}~\cite{xeon-4215} & 14 nm & 8 (16 threads) & 2.5 GHz & 40 GFLOPS$^\star$ & 256 GB & 37.5 GB/s & 85 W \\ \hline
\textbf{NVIDIA A100 GPU}~\cite{a100} & 7 nm & 108 (6,912 SIMD lanes) & 1.4 GHz & 19,500 GFLOPS & 40 GB & 1555 GB/s & 250 W \\ \hline
%\textbf{NVIDIA Titan V GPU}~\cite{titanv} & 14 nm & 80 (5,120 SIMD lanes) & 1.2 GHz & 12,288 GFLOPS & 12 GB & 652.8 GB/s & 250 W \\ \hline
%\textbf{Intel Xeon E3-1225 v6 CPU}~\cite{xeon-e3-1225} & 14 nm & 4 (8 threads) & 3.3 GHz & 26.4 GFLOPS$^\star$ & 32 GB & 37.5 GB/s & 73 W \\ \hline
%\textbf{640-DPU PIM System} & 2x nm & 640 & 267 MHz & 170.9 GOPS & 40 GB & 333.75 GB/s & 96 W$^\dagger$ \\ \hline
\end{tabular}


==> UPMEM+ML - ISVLSI - arXiv-2/figures/tab-datasets.tex <==
\begin{tabular}{|l||l|l|l|}
\hline
\multirow{2}{*}{\textbf{ML Workload}} & \multicolumn{2}{c|}{\textbf{Synthetic Datasets}} & \multirow{2}{*}{\textbf{Real Dataset}} \\
\cline{2-3}
  & \textbf{Strong Scaling (1 PIM core | 256-2048 PIM cores)} & \textbf{Weak Scaling (per PIM core)} &   \\
\hline
\hline
Linear regression & 2,048 samples, 16 attr. (0.125 MB) | 6,291,456 samples, 16 attr. (384 MB) & 2,048 samples, 16 attr. (0.125 MB) & SUSY~\cite{baldi2014searching, susy} \\ \hline
Logistic regression & 2,048 samples, 16 attr. (0.125 MB) | 6,291,456 samples, 16 attr. (384 MB) & 2,048 samples, 16 attr. (0.125 MB) & Skin segmentation~\cite{skin} \\ \hline
Decision tree & 60,000 samples, 16 attr. (3.84 MB) | 153,600,000 samples, 16 attr. (9830 MB) & 600,000 samples, 16 attr. (38.4 MB) & Higgs boson~\cite{baldi2014searching, Dua:2019} \\ \hline
K-Means & 10,000 samples, 16 attr. (0.64 MB) | 25,600,000 samples, 16 attr. (1640 MB) & 100,000 samples, 16 attr. (6.4 MB) & Higgs boson~\cite{baldi2014searching, Dua:2019} \\ \hline
\end{tabular}


==> UPMEM+ML - ISVLSI - arXiv-2/figures/tab-diversity.tex <==
\begin{tabular}{|l|l|l|c||c|c|c|c|c|c|c|}
    \hline
    \textbf{Learning} & \multirow{2}{*}{\textbf{Application}} & \multirow{2}{*}{\textbf{Algorithm}} & \multirow{2}{*}{\textbf{Short name}} & \multicolumn{3}{c|}{\textbf{Memory access pattern}} & \multicolumn{2}{c|}{\textbf{Computation pattern}} & \multicolumn{2}{c|}{\textbf{Communication/synchronization}}  \\
    \cline{5-11}
     \textbf{approach} & & & & \textbf{Sequential} & \textbf{Strided} & \textbf{Random} & \textbf{Operations} & \textbf{Datatype} & \textbf{Intra PIM Core} & \textbf{Inter PIM Core}  \\
    \hline
    \hline
    \multirow{3}{*}{Supervised}
      & Regression & \textbf{Linear Regression} & \texttt{LIN} & Yes & No & No & mul, add & float, int32\_t & barrier & Yes \\
    \cline{2-11}
      & \multirow{2}{*}{Classification} & \textbf{Logistic Regression} & \texttt{LOG} & Yes & No & No & mul, add, exp, div & float, int32\_t & barrier & Yes \\
    \cline{3-11}
      & & \textbf{Decision Tree} & \texttt{DTR} & Yes & No & No & compare, add & float & barrier, mutex & Yes \\
    \hline
    \multirow{1}{*}{Unsupervised}
      & Clustering & \textbf{K-Means} & \texttt{KME} & Yes & No & No & mul, compare, add  & int16\_t, int64\_t & barrier, mutex & Yes \\
    \hline
\end{tabular}


==> UPMEM+ML - ISVLSI - arXiv-2/figures/tab-dtr.tex <==
\begin{tabular}{|l|l||c|}
\hline
\textbf{ML workload} & \textbf{Version} & \textbf{Training accuracy} \\
\hline
\hline
\multirow{3}{*}{Decision tree} & \texttt{DTR} (PIM) & 0.65635 \\ \cline{2-3}
& CPU~\cite{pedregosa2011scikit} & 0.65581 \\ \cline{2-3}
& GPU~\cite{rapids} & 0.70462 \\ \hline
\end{tabular}


==> UPMEM+ML - ISVLSI - arXiv-2/figures/tab-kme.tex <==
\begin{tabular}{|l|l||c|}
\hline
\textbf{ML workload} & \textbf{Version} & \textbf{Adjusted Rand index} \\
\hline
\hline
\multirow{3}{*}{K-means} & \texttt{KME} (PIM) & 0.999985 \\ \cline{2-3}
& CPU~\cite{pedregosa2011scikit} & 1 \\ \cline{2-3}
& GPU~\cite{rapids} & 0.758579 \\ \hline
\end{tabular}


==> UPMEM+ML - ISVLSI - arXiv-2/figures/tab-linlog-error.tex <==
\begin{tabular}{|l|l||c|}
\hline
\textbf{ML workload} & \textbf{Version} & \textbf{Training error rate (\%)} \\
\hline
\hline
\multirow{6}{*}{Linear regression} & \texttt{LIN-FP32} & 13.88 \\ \cline{2-3}
& \texttt{LIN-INT32} & 18.68 \\ \cline{2-3}
& \texttt{LIN-HYB} & 18.68 \\ \cline{2-3}
& \texttt{LIN-BUI} & 18.68 \\ \cline{2-3}
& CPU~\cite{mkl} & 13.88 \\ \cline{2-3}
& GPU~\cite{cublas} & 13.88 \\ \hline
\multirow{8}{*}{Logistic regression} & \texttt{LOG-FP32} & 7.58 \\ \cline{2-3}
& \texttt{LOG-INT32} & 8.72 \\ \cline{2-3}
& \texttt{LOG-INT32-LUT (MRAM)} & 8.72 \\ \cline{2-3}
& \texttt{LOG-INT32-LUT (WRAM)} & 8.98 \\ \cline{2-3}
& \texttt{LOG-HYB-LUT (WRAM)} & 8.98 \\ \cline{2-3}
& \texttt{LOG-BUI-LUT (WRAM)} & 8.98 \\ \cline{2-3}
& CPU~\cite{mkl} & 7.58 \\ \cline{2-3}
& GPU~\cite{cublas} & 7.58 \\ \hline
\end{tabular}


==> UPMEM+ML - ISVLSI - arXiv-2/sections/01-introduction.tex <==
%\section{Introduction}

%Importance of machine learning workloads and massive amounts of data in training. Huge training datasets. 
%Motivation: How data movement bottleneck affects ML workloads. Motivate with recent characterization works.
%CPUs and GPUs achieve sustained throughput that is far from peak due to memory access intensity.
Machine learning (ML) algorithms~\cite{geron2019, alpaydin2020, goodfellow2016, mohri2018, shalev2014, raschka2019} have become ubiquitous in many fields of science and technology due to their ability to learn \juan{from} and %enhance from 
\juan{improve with} experience with minimal human intervention. These algorithms train by updating their model parameters in an iterative manner to improve the overall prediction accuracy.  %their innumerable applications. 
However, training machine learning algorithms is a computationally intensive process, which requires large amounts of training data. 
Accessing training data in current processor-centric systems (e.g., CPU, GPU) implies costly data movement between memory and processors, which results in high energy consumption and a large percentage of the total execution cycles. 
This data movement can become the bottleneck of the training process, if there is not enough computation and locality to amortize its cost. 

%PIM is a promising direction. 
%Quick overview of recent PIM architectures.
One way to alleviate the cost of data movement is \emph{processing-in-memory} (\emph{PIM})~\cite{mutlu2019,mutlu2020modern, ghoseibm2019, seshadri2020indram, mutlu2019enabling}, a \juan{data-centric} computing paradigm that places processing elements near or inside the memory arrays. 
PIM has been explored for decades~\cite{stone1970logic, Kautz1969, shaw1981non, kogge1994, gokhale1995processing, patterson1997case, oskin1998active, kang1999flexram, Mai:2000:SMM:339647.339673,murphy2001characterization, Draper:2002:ADP:514191.514197,aga.hpca17,eckert2018neural,fujiki2019duality,kang.icassp14,seshadri.micro17,seshadri.arxiv16,Seshadri:2015:ANDOR,seshadri2013rowclone,angizi2019graphide,kim.hpca18,kim.hpca19,gao2020computedram,chang.hpca16,xin2020elp2im,li.micro17,deng.dac2018,hajinazarsimdram,rezaei2020nom,wang2020figaro,ali2019memory,li.dac16,angizi2018pima,angizi2018cmp,angizi2019dna,levy.microelec14,kvatinsky.tcasii14,shafiee2016isaac,kvatinsky.iccd11,kvatinsky.tvlsi14,gaillardon2016plim,bhattacharjee2017revamp,hamdioui2015memristor,xie2015fast,hamdioui2017myth,yu2018memristive,syncron,fernandez2020natsa,cali2020genasm,kim.bmc18,ahn.pei.isca15,ahn.tesseract.isca15,boroumand.asplos18,boroumand2019conda,singh2019napel,asghari-moghaddam.micro16,DBLP:conf/sigmod/BabarinsaI15,chi2016prime,farmahini2015nda,gao.pact15,DBLP:conf/hpca/GaoK16,gu.isca16,guo2014wondp,hashemi.isca16,cont-runahead,hsieh.isca16,kim.isca16,kim.sc17,DBLP:conf/IEEEpact/LeeSK15,liu-spaa17,morad.taco15,nai2017graphpim,pattnaik.pact16,pugsley2014ndc,zhang.hpdc14,zhu2013accelerating,DBLP:conf/isca/AkinFH15,gao2017tetris,drumond2017mondrian,dai2018graphh,zhang2018graphp,huang2020heterogeneous,zhuo2019graphq,santos2017operand,ghoseibm2019,wen2017rebooting,besta2021sisa,ferreira2021pluto,olgun2021quactrng,lloyd2015memory,elliott1999computational,zheng2016tcam,landgraf2021combining,rodrigues2016scattergather,lloyd2018dse,lloyd2017keyvalue,gokhale2015rearr,nair2015active,jacob2016compiling,sura2015data,nair2015evolution,balasubramonian2014near,xi2020memory,impica,boroumand2016pim,giannoula2022sparsep,giannoula2022sigmetrics,denzler2021casper,boroumand2021polynesia,boroumand2021icde,singh2021fpga,singh2021accelerating,herruzo2021enabling,yavits2021giraf,asgarifafnir,boroumand2021google_arxiv,boroumand2021google,amiraliphd,singh2020nero,seshadri.bookchapter17,diab2022high,diab2022hicomb,fujiki2018memory,zha2020hyper,mutlu.imw13,mutlu.superfri15,ahmed2019compiler,jain2018computing,ghiasi2022genstore,deoliveira2021IEEE,deoliveira2021,cho2020mcdram,shin2018mcdram,gu2020ipim,lavenier2020,Zois2018}. However, memory technology challenges prevented from its successful materialization in commercial products. For example, the limited number of metal layers in DRAM~\cite{weber2005current,peng2015design} makes conventional processor designs %unfeasible
\juang{impractical} \juan{in commodity DRAM chips}~\cite{devaux2019,yuffe2011,christy2020,singh2017}.

%Only recently the first 
\juan{Real-world} PIM systems have %appeared
\juan{only recently been manufactured and commercialized}. 
The UPMEM company, for example, %commercializes 
\juan{introduced} the first general-purpose \juan{commercial} PIM architecture~\cite{upmem,upmem2018,gomezluna2021benchmarking, gomezluna2022ieeeaccess, gomezluna2021cut}, which integrates small in-order cores near DRAM memory banks. 
High-bandwidth memory (HBM)-based HBM-PIM~\cite{kwon202125, lee2021hardware} and Acceleration DIMM (AxDIMM)~\cite{ke2021near} are Samsung's proposals that have been successfully tested %on 
\juan{via real} prototypes. HBM-PIM features \emph{Single Instruction Multiple Data} (\emph{SIMD}) units, which %compute 
\juan{support} multiply-add and multiply-accumulate operations, near the banks in HBM layers~\cite{jedec.hbm.spec, lee.taco16}, and it is designed to accelerate neural network inference. AxDIMM is a near-rank solution that places an FPGA fabric on \juan{a DDR module} %DIMMs 
to accelerate specific workloads (e.g., recommendation inference). 
Accelerator-in-Memory (AiM)~\cite{lee2022isscc} is a GDDR6-based PIM architecture from SK Hynix with specialized units for multiply-accumulate and activation functions for deep learning. 
HB-PNM~\cite{niu2022isscc} is a 3D-stacked-based PIM architecture from Alibaba, which stacks a layer of LPDDR4 memory and a logic layer with specialized accelerators for \juan{recommendation} systems.

\juan{These five real-world PIM systems} %architectures 
have some important \juan{common} characteristics, \juan{as depicted in Figure~\ref{fig:scheme}}. %in common. 
First, there is a host processor (CPU or GPU), typically with a deep cache hierarchy, which has access to (1) standard main memory, and (2) PIM-enabled memory (i.e., UPMEM DIMMs, HBM-PIM stacks, AxDIMM DIMMs, AiM GDDR6, HB-PNM LPDDR4). 
Second, the PIM-enabled memory \juan{chip} contains multiple PIM processing elements (PIM PEs), which have access to memory (either memory banks or ranks) with higher %(aggregated) 
bandwidth \juan{and lower latency} than the host processor. 
Third, the \juan{PIM} processing elements (either \juan{general-purpose} cores, SIMD \juan{units, FPGAs, or specialized processors}) run at \juang{only} a few hundred megahertz, and have a small number of registers and %a little 
\juan{relatively small} (or no) cache or scratchpad memory. 
Fourth, processing elements may not be able to communicate directly \juan{with each other} (e.g., UPMEM DPUs, HBM-PIM PCUs or AiM PUs in different chips), %so that 
\juan{and} communication \juan{between them} happens via the host processor. %\todo{GERALDO: Revise this sentence which may not be true for HBM-PIM, AiM, HB-PNM}. 
Figure~\ref{fig:scheme} shows a high-level view of such a state-of-the-art processing-in-memory system. 

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{figures/PIM-system-v2.pdf}
\caption{High-level view of a state-of-the-art processing-in-memory system. \juan{The host CPU has access to $M$ standard memory modules and $N$ PIM-enabled memory modules.}}
\label{fig:scheme}
\end{figure}


%Goal. Focus on clustering and classification. 
Our goal in this work is to quantify the potential of general-purpose PIM architectures for training of machine learning algorithms. 
To this end, we implement four representative \juan{classical} machine learning algorithms (linear regression~\cite{freedman2009statistical, yan2009linear}, logistic regression~\cite{freedman2009statistical, hosmer2013applied}, decision tree~\cite{suthaharan2016decision}, K-means clustering~\cite{Lloyd82leastsquares}) %for 
\juan{on} a general-purpose memory-centric system containing PIM-enabled memory, % with 
\juan{specifically} the UPMEM PIM architecture~\cite{upmem,upmem2018,gomezluna2021benchmarking, gomezluna2022ieeeaccess, gomezluna2021cut}. 
We do \emph{not} include training of deep learning %(DL) 
algorithms in our study, since GPUs \juan{and TPUs} have a solid position as the preferred \juan{and highly optimized accelerators for %DL
deep learning} training~\cite{hwukirk2016.nn,chetlur2014cudnn,gao2017tetris,abadi2016tensorflow,runai_gpu,jouppi2017datacenter, jouppi2021ten}. 

Our PIM implementations of ML algorithms follow \juan{PIM} programming recommendations in recent literature~\cite{upmem-guide, upmem2018, gomezluna2021benchmarking, gomezluna2022ieeeaccess}. 
We apply several optimizations to overcome the limitations of existing general-purpose PIM architectures (e.g., limited instruction set, relatively simple pipeline, relatively low frequency) and take full advantage of the inherent strengths of PIM (e.g., large memory bandwidth, \juan{low memory latency}). 

We evaluate our PIM implementations in terms of \juang{training} accuracy, performance, and scaling characteristics on a \juan{real} memory-centric system with PIM-enabled memory~\cite{upmem, upmem-sdk, upmem-guide}. 
\juan{We run our experiments on a real-world PIM system~\cite{upmem} with 2,524 PIM cores running at 425 MHz, and 158 GB of DRAM memory.\footnote{The UPMEM-based PIM system has up to 2,560 PIM cores and 160 GB of DRAM.}}

Our experimental \juan{real system} evaluation provides %interesting 
\juan{new} observations and insights, %such as the following ones:
\juan{including the following:} 
\begin{itemize}
\item ML training workloads that %are memory-bound 
\juan{show memory-bound behavior} in processor-centric systems can greatly benefit from (1) fixed-point \juang{data} representation, (2) quantization~\cite{zmora2021quantization,gholamisurvey}, and (3) hybrid precision implementation~\cite{hopper, lee2022isscc} \juan{(without much accuracy loss) in PIM systems}, in order to %palliate 
\juan{alleviate} the lack of native support for floating-point %operands 
%\juan{operations} 
and high-precision (i.e., 32- and 64-bit) \juang{arithmetic operations}. 
\item ML training workloads that require complex activation functions (e.g., sigmoid)~\cite{han1995influence} can take advantage of \emph{lookup tables} (\emph{LUTs})~\cite{ferreira2021pluto, deng2019lacc, gao2016draf} \juan{in PIM systems} instead of function approximation (e.g., Taylor series)~\cite{weisstein2004taylor}, when %they 
\juan{PIM systems} lack native support for those activation functions. 
\item %Data layout can be arranged in a way that 
\juan{Data can be placed and laid out such that} accesses of PIM cores to their nearby memory banks are %in 
streaming, %thus providing 
\juan{which enables} better exploitation of the \juan{PIM} memory bandwidth. 
\item ML training workloads with large training datasets can greatly benefit from scaling \juan{the size of} PIM-enabled memory with PIM cores attached to memory banks. Training datasets can remain in memory without being moved to the host processor (e.g., CPU, GPU) in every iteration of the training process. Even if PIM cores need to communicate intermediate results via the host processor, this communication overhead is %easily 
tolerable \juan{with proper overlap of computation and communication}. 
\end{itemize}


%\jgl{Optimizations for distributed system: pipelining, overlapping of transfers and computation.}\\
%Optimizations that are enabled by PIM nature: LUTs...\\
%Optimizations that target specific hardware limitations: int8/hybrid...
%Data reordering for streaming accesses (better exploitation of the internal bandwidth).

%We evaluate the ML workloads in terms of quality, performance and scaling characteristics. 
%We evaluate our implementations on a large PIM-enabled system. 

We compare our PIM implementations of linear regression, \juan{logistic} regression, decision tree, and K-means clustering to their state-of-the-art CPU and GPU counterparts. We observe that memory-centric systems with PIM-enabled memory can significantly outperform processor-centric systems for memory-bound ML training workloads, when the operations needed by the ML workloads are natively supported by PIM hardware (or can be replaced by \juan{efficient LUT implementations}). % queries). 

Our extended paper~\cite{gomez2022experimental} contains (1) detailed description of our PIM implementations of ML workloads; (2) comprehensive evaluation and \juang{comparisons to state-of-the-art CPU and GPU systems}; and (3) more insights about the suitability of ML workloads to the PIM system, programming recommendations for ML software developers, and suggestions and hints for future PIM architectures. 
We \juan{aim to} open-source all our PIM implementations of ML training workloads, training datasets, and evaluation scripts.


==> figures/tab-comparison.tex <==
\begin{tabular}{|l||l|l|}
\hline
\textbf{ML workload} & \textbf{CPU implementation} & \textbf{GPU implementation} \\
\hline
\hline
Linear regression & Intel MKL~\cite{mkl} & NVIDIA cuBLAS~\cite{cublas} \\ \hline
Logistic regression & Intel MKL~\cite{mkl} & NVIDIA cuBLAS~\cite{cublas} \\ \hline
Decision tree & Scikit-learn~\cite{pedregosa2011scikit} & RAPIDS~\cite{rapids} \\ \hline
Kmeans & Scikit-learn~\cite{pedregosa2011scikit} & RAPIDS~\cite{rapids} \\ \hline
\end{tabular}


==> figures/tab-cpugpu.tex <==
\begin{tabular}{|l||c|ccc|cc|c|}
\hline
\multirow{2}{*}{\textbf{System}} & \textbf{Process} & \multicolumn{3}{c|}{\textbf{Processor Cores}} & \multicolumn{2}{c|}{\textbf{Memory}} & \multirow{2}{*}{\textbf{TDP}} \\
\cline{3-7}
& \textbf{Node} & \textbf{Total Cores} & \textbf{Frequency} & \textbf{Peak Performance} & \textbf{Capacity} & \textbf{Total Bandwidth} & \\
\hline
\hline
\textbf{UPMEM PIM System}~\cite{upmem} & 2x nm & 2,560$^\diamond$ & 425 MHz & 1,088 GOPS & 160 GB & 2.1 TB/s & 280 W$^\dagger$ \\ \hline
\textbf{Intel Xeon Silver 4215 CPU}~\cite{xeon-4215} & 14 nm & 8 (16 threads) & 2.5 GHz & 40 GFLOPS$^\star$ & 256 GB & 37.5 GB/s & 85 W \\ \hline
\textbf{NVIDIA A100 GPU}~\cite{a100} & 7 nm & 108 (6,912 SIMD lanes) & 1.4 GHz & 19,500 GFLOPS & 40 GB & 1555 GB/s & 250 W \\ \hline
%\textbf{NVIDIA Titan V GPU}~\cite{titanv} & 14 nm & 80 (5,120 SIMD lanes) & 1.2 GHz & 12,288 GFLOPS & 12 GB & 652.8 GB/s & 250 W \\ \hline
%\textbf{Intel Xeon E3-1225 v6 CPU}~\cite{xeon-e3-1225} & 14 nm & 4 (8 threads) & 3.3 GHz & 26.4 GFLOPS$^\star$ & 32 GB & 37.5 GB/s & 73 W \\ \hline
%\textbf{640-DPU PIM System} & 2x nm & 640 & 267 MHz & 170.9 GOPS & 40 GB & 333.75 GB/s & 96 W$^\dagger$ \\ \hline
\end{tabular}


==> figures/tab-datasets.tex <==
\begin{tabular}{|l||l|l|l|}
\hline
\multirow{2}{*}{\textbf{ML Workload}} & \multicolumn{2}{c|}{\textbf{Synthetic Datasets}} & \multirow{2}{*}{\textbf{Real Dataset}} \\
\cline{2-3}
  & \textbf{Strong Scaling (1 PIM core | 256-2048 PIM cores)} & \textbf{Weak Scaling (per PIM core)} &   \\
\hline
\hline
Linear regression & 2,048 samples, 16 attr. (0.125 MB) | 6,291,456 samples, 16 attr. (384 MB) & 2,048 samples, 16 attr. (0.125 MB) & SUSY~\cite{baldi2014searching, susy} \\ \hline
Logistic regression & 2,048 samples, 16 attr. (0.125 MB) | 6,291,456 samples, 16 attr. (384 MB) & 2,048 samples, 16 attr. (0.125 MB) & Skin segmentation~\cite{skin} \\ \hline
Decision tree & 60,000 samples, 16 attr. (3.84 MB) | 153,600,000 samples, 16 attr. (9830 MB) & 600,000 samples, 16 attr. (38.4 MB) & Higgs boson~\cite{baldi2014searching, Dua:2019} \\ \hline
K-Means & 10,000 samples, 16 attr. (0.64 MB) | 25,600,000 samples, 16 attr. (1640 MB) & 100,000 samples, 16 attr. (6.4 MB) & Higgs boson~\cite{baldi2014searching, Dua:2019} \\ \hline
\end{tabular}


==> figures/tab-diversity.tex <==
\begin{tabular}{|l|l|l|c||c|c|c|c|c|c|c|}
    \hline
    \textbf{Learning} & \multirow{2}{*}{\textbf{Application}} & \multirow{2}{*}{\textbf{Algorithm}} & \multirow{2}{*}{\textbf{Short name}} & \multicolumn{3}{c|}{\textbf{Memory access pattern}} & \multicolumn{2}{c|}{\textbf{Computation pattern}} & \multicolumn{2}{c|}{\textbf{Communication/synchronization}}  \\
    \cline{5-11}
     \textbf{approach} & & & & \textbf{Sequential} & \textbf{Strided} & \textbf{Random} & \textbf{Operations} & \textbf{Datatype} & \textbf{Intra PIM Core} & \textbf{Inter PIM Core}  \\
    \hline
    \hline
    \multirow{3}{*}{Supervised}
      & Regression & \textbf{Linear Regression} & \texttt{LIN} & Yes & No & No & mul, add & float, int32\_t & barrier & Yes \\
    \cline{2-11}
      & \multirow{2}{*}{Classification} & \textbf{Logistic Regression} & \texttt{LOG} & Yes & No & No & mul, add, exp, div & float, int32\_t & barrier & Yes \\
    \cline{3-11}
      & & \textbf{Decision Tree} & \texttt{DTR} & Yes & No & No & compare, add & float & barrier, mutex & Yes \\
    \hline
    \multirow{1}{*}{Unsupervised}
      & Clustering & \textbf{K-Means} & \texttt{KME} & Yes & No & No & mul, compare, add  & int16\_t, int64\_t & barrier, mutex & Yes \\
    \hline
\end{tabular}


==> figures/tab-dtr.tex <==
\begin{tabular}{|l|l||c|}
\hline
\textbf{ML workload} & \textbf{Version} & \textbf{Training accuracy} \\
\hline
\hline
\multirow{3}{*}{Decision tree} & \texttt{DTR} (PIM) & 0.65635 \\ \cline{2-3}
& CPU~\cite{pedregosa2011scikit} & 0.65581 \\ \cline{2-3}
& GPU~\cite{rapids} & 0.70462 \\ \hline
\end{tabular}


==> figures/tab-kme.tex <==
\begin{tabular}{|l|l||c|}
\hline
\textbf{ML workload} & \textbf{Version} & \textbf{Adjusted Rand index} \\
\hline
\hline
\multirow{3}{*}{K-means} & \texttt{KME} (PIM) & 0.999985 \\ \cline{2-3}
& CPU~\cite{pedregosa2011scikit} & 1 \\ \cline{2-3}
& GPU~\cite{rapids} & 0.758579 \\ \hline
\end{tabular}


==> figures/tab-linlog-error.tex <==
\begin{tabular}{|l|l||c|}
\hline
\textbf{ML workload} & \textbf{Version} & \textbf{Training error rate (\%)} \\
\hline
\hline
\multirow{6}{*}{Linear regression} & \texttt{LIN-FP32} & 13.88 \\ \cline{2-3}
& \texttt{LIN-INT32} & 18.68 \\ \cline{2-3}
& \texttt{LIN-HYB} & 18.68 \\ \cline{2-3}
& \texttt{LIN-BUI} & 18.68 \\ \cline{2-3}
& CPU~\cite{mkl} & 13.88 \\ \cline{2-3}
& GPU~\cite{cublas} & 13.88 \\ \hline
\multirow{8}{*}{Logistic regression} & \texttt{LOG-FP32} & 7.58 \\ \cline{2-3}
& \texttt{LOG-INT32} & 8.72 \\ \cline{2-3}
& \texttt{LOG-INT32-LUT (MRAM)} & 8.72 \\ \cline{2-3}
& \texttt{LOG-INT32-LUT (WRAM)} & 8.98 \\ \cline{2-3}
& \texttt{LOG-HYB-LUT (WRAM)} & 8.98 \\ \cline{2-3}
& \texttt{LOG-BUI-LUT (WRAM)} & 8.98 \\ \cline{2-3}
& CPU~\cite{mkl} & 7.58 \\ \cline{2-3}
& GPU~\cite{cublas} & 7.58 \\ \hline
\end{tabular}

